Protocol-based Smart Contract Generation

The popularity of smart contracts is on the rise, yet breaches in reliability and security linger. Among the many facets of smart contract reliability, we concentrate on faults rooted in out-of-order interactions with contract endpoints. We propose SmartScribble, a protocol language to describe valid patterns of interaction between users and endpoints. SmartScribble not only ensures correct interactive behaviour but also simplifies smart contract coding. From a protocol description, our compiler generates a smart contract that can then be completed by the programmer with the relevant business logic. The generated contracts rely on finite state machines to control endpoint invocations. As a proof of concept, we target Plutus, the contract programming language for the Cardano blockchain. Preliminary evaluation points to a 75% decrease in the size of the code that developers must write, coupled with an increase of reliability by enforcing the specified patterns of interaction.

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Blockchain providers are focused on the development of programming languages relying on formal verification. Examples are Liquidity (by Tezos) [3], Plutus (by IOHK) [19], Move (by Facebook) [11], or Rholang (by RChain) [4]. These languages rely on expressive types to specify safety properties. As future work, we plan to incorporate session types to model the \ourlanguage\ protocols and provide stronger guarantees on the correctness of contract execution.

Several programming languages for smart contracts have been proposed in the last few years. The smart contract language that, currently, seems closer to \ourlanguage\ is FSolidM~\cite{Mavridou2017}. Mavridou and Laszka proposed a model for smart contracts based on finite state machines. While their approach relies on the explicit construction of finite state machines for contract's specification, we only used state machines as  auxiliary data structures to test our proposed language. We plan to capitalize on the parallel between Scribble and session types~\cite{yoshida2013scribble,Yoshida2014} and delegate the protocol's execution control on session types~\cite{honda1998language,vasconcelos2012fundamentals}. The basic premise underlying a smart contract matches the primary motivation for session types: ensure compliance with protocols. Session types extend traditional types by enabling to capture protocol interactions in the types~\cite{honda1998language,vasconcelos2012fundamentals}. Among the many proposals of smart contract languages, there are domain-specific languages, such as BitML that is integrated with the Bitcoin blockhain~\cite{Bartoletti2018}, typestate-oriented languages such as Obsidian~\cite{coblenz2020obsidian}, and functional (session-typed) languages, such as Nomos~\cite{nomos}. 


%
%the description of an overall behaviour of a set of components and interactions
%that are guaranteed to satisfy a global strategy~\cite{Bartoletti2020}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../protocol_based_SC_generation"
%%% End:

